Syfer: Neural Obfuscation for Private Data Release

Balancing privacy and predictive utility remains a central challenge for machine learning in healthcare. In this paper, we develop Syfer, a neural obfuscation method to protect against re-identification attacks. Syfer composes trained layers with random neural networks to encode the original data (e.g. X-rays) while maintaining the ability to predict diagnoses from the encoded data. The randomness in the encoder acts as the private key for the data owner. We quantify privacy as the number of attacker guesses required to re-identify a single image (guesswork). We propose a contrastive learning algorithm to estimate guesswork. We show empirically that differentially private methods, such as DP-Image, obtain privacy at a significant loss of utility. In contrast, Syfer achieves strong privacy while preserving utility. For example, X-ray classifiers built with DP-image, Syfer, and original data achieve average AUCs of 0.53, 0.78, and 0.86, respectively.

==> intro-new.tex <==
\section{Introduction}


Data sharing is a key bottleneck for the development of equitable clinical AI algorithms.
Public medical datasets are constrained by privacy regulations like HIPAA~\cite{HIPAA} and GDPR~\cite{GDPR}, that aim to prevent leakage of identifiable patient data.

In this paper, we propose a novel framework where data owners encode their data with a random neural network and apply a random permutation to the label identities.
The randomly encoded dataset is then released, with the data owner's random choices (e.g. sampling of random weights) serving as their private key.
A successful scheme should support model development on any downstream tasks using standard machine learning tools, while still preventing attackers without the private key from re-identifying raw samples.

Increasingly significant research efforts in developing privacy-preserving machine learning methods have proved succesful: current methods, such as differential privacy and homomorphic encryption, provide strong universal privacy guarantees but do so by sacrificing the predictive utility of the data they wish to protect.
In this work, we hypothesize that we can learn
learning how to encode
specific data distribution

Our threat model considers an adversary with knowledge of the raw image distribution, the released encoded data and the randomized encoding scheme.
While the adversary can simulate the randomized encoding scheme, they do not have access to the data owner's particular choice of randomness, which serves as a private key.
We measure the privacy of an encoding scheme as its guesswork, i.e. the number of guesses an attacker requires to match a single raw image to its corresponding encoded sample. A guesswork of one implies that an attacker can confidently identify at least a single patient from the encoded data, violating the privacy notions of HIPAA, and a high guesswork means that an attacker cannot confidently identify any sample.

We estimate the privacy of an encoding scheme on a particular dataset using a model-based attacker. This attacker is implemented as a contrastive learning algorithm, which is trained to maximize the likelihood of re-identifying raw images across encodings. In our setting, the attacker has access to both the raw images and the encoded images and only needs to predict the matching between corresponding pairs. This extreme setup acts as a lower bound on the scheme's privacy in a real-world setting, where the attacker's knowledge of the raw images is imperfect.

We trained \name on a public X-ray dataset from NIH, and evaluated the privacy and utility of the scheme on heldout dataset (MIMIC-CXR) across multiple attacker architectures and prediction tasks. We found that \name obtained strong privacy, with a guesswork of 8411, i.e., it takes an attacker with an access to an oracle an average of 8411 guesses to correctly guess a raw~image--encoded~image correspondence. Moreover, models built on \name encodings approached the accuracy of models built on raw images, obtaining an average AUC of 78 across diagnosis tasks compared to 84 by a non-private baseline with the same architecture, and 86 by the best raw-image baseline. In contrast, prior encoding schemes, like InstaHide~\cite{instahide} and Dauntless~\cite{DAUnTLeSS}, do not meet our privacy requirements, achieving both a guesswork of 1. While differential privacy schemes, such as DP-Image~\cite{liu2021dp}, can eventually meet our privacy standard with large enough noise, achieving a guesswork of 1379, this results in too large of a utility loss, i.e. an AUC of 53.







==> table <==
\hline
Dauntless          & $1.0 $  $(1, 1)       $ & $1.00$ $(1.00, 1.00)$ \\
InstaHide          & $1.0 $  $(1, 1)       $ & $1.00$ $(1.00, 1.00)$ \\
DP-S, $b=10$       & $1.2 $  $(1, 2)       $ & $0.98 $ $(0.98, 0.98)  $\\
DP-S, $b=20$       & $7.2 $  $(1, 31)      $ & $0.86 $ $(0.85, 0.86)  $\\
DP-S, $b=30$       & $68  $  $(1, 205)     $ & $0.70 $ $(0.70, 0.70)  $\\
DP-I, $b=1$        & $5.0 $  $(1, 17)      $ & $0.89 $ $(0.88, 0.89)  $\\
DP-I, $b=3$        & $77  $  $(3, 276)     $ & $0.73 $ $(0.73, 0.73)  $\\
DP-I, $b=5$        & $1379$  $(49, 4135)   $ & $0.59 $ $(0.59, 0.60)  $\\
\name-Random       & $1.7 $  $(1, 4)       $ & $0.99 $ $(0.99, 0.99) $\\
\name ($T^X$ only) & $8476$  $(1971, 20225)$ & $0.50 $ $(0.49, 0.52) $\\
\hline


SAU       & $8476 $ $(1971, 20225)$ & $0.50$ $(0.49, 0.52)$ \\
ViT       & $8411 $ $(5219, 12033)$ & $0.50$ $(0.49, 0.51)$ \\
Resnet-18 & $10070$ $(9871, 10300)$ & $0.50$ $(0.47, 0.53)$  	 \\

Edema         & $3617 $ $(94, 11544)  $  & $0.50$ $(0.49, 0.51)$\\
Consolidation & $1697 $ $(83, 5297)   $  & $0.55$ $(0.53, 0.57)$ \\
Cardiomegaly  & $9834 $ $(2072, 15766)$  & $0.51$ $(0.49, 0.53)$ \\
Atelectasis   & $13189$ $(2511, 28171)$  & $0.50$ $(0.48, 0.52)$ \\

Edema         & $47$ $(12, 83)$ & $0.76$ $(0.76, 0.76)$ \\
Consolidation & $36$ $(2, 104)$ & $0.76$ $(0.76, 0.76)$\\
Cardiomegaly  & $42$ $(17, 57)$ & $0.75$ $(0.75, 0.75)$ \\
Atelectasis   & $80$ $(65, 98)$ & $0.75$ $(0.75, 0.75)$ \\


Plaintext         & $0.91$ & $0.78$ & $0.89$ & $0.85$ & $0.86$\\
DP-Simple, $b=10$ & $0.51$ & $0.51$ & $0.52$ & $0.52$ & $0.52$\\
DP-Simple, $b=20$ & $0.50$ & $0.50$ & $0.50$ & $0.50$ & $0.50$\\
DP-Simple, $b=30$ & $0.49$ & $0.49$ & $0.50$ & $0.51$ & $0.50$\\
DP-Image, $b=1$   & $0.60$ & $0.59$ & $0.60$ & $0.59$ & $0.60$\\
DP-Image, $b=2$   & $0.54$ & $0.50$ & $0.55$ & $0.55$ & $0.54$\\
DP-Image, $b=5$   & $0.53$ & $0.55$ & $0.51$ & $0.52$ & $0.53$\\
\name-Random      & $0.89$ & $0.75$ & $0.86$ & $0.84$ & $0.84$\\
\name             & $0.82$ & $0.69$ & $0.81$ & $0.78$ & $0.78$\\

----

\hline
Dauntless          & $1.0 $  $(1, 1)       $ & $100$ $(100, 100)$ \\
InstaHide          & $1.0 $  $(1, 1)       $ & $100$ $(100, 100)$ \\
DP-S, $b=10$       & $1.2 $  $(1, 2)       $ & $98 $ $(98, 98)  $\\
DP-S, $b=20$       & $7.2 $  $(1, 31)      $ & $86 $ $(85, 86)  $\\
DP-S, $b=30$       & $68  $  $(1, 205)     $ & $70 $ $(70, 70)  $\\
DP-I, $b=1$        & $5.0 $  $(1, 17)      $ & $89 $ $(88, 89)  $\\
DP-I, $b=3$        & $77  $  $(3, 276)     $ & $73 $ $(73, 73)  $\\
DP-I, $b=5$        & $1379$  $(49, 4135)   $ & $59 $ $(59, 60)  $\\
\name-Random       & $1.7 $  $(1, 4)       $ & $99 $ $(99, 99) $\\
\name ($T^X$ only) & 8476 $  $(1971, 20225)$ & $50 $ $(49, 52) $\\
\hline


SAU       & $8476 $ $(1971, 20225)$ & $50$ $(49, 52)$ \\
ViT       & $8411 $ $(5219, 12033)$ & $50$ $(49, 51)$ \\
Resnet-18 & $10070$ $(9871, 10300)$ & $50$ $(47, 53)$  	 \\

Edema         & $3617 $ $(94, 11544)  $  & $50$ $(49, 51)$\\
Consolidation & $1697 $ $(83, 5297)   $  & $55$ $(53, 57)$ \\
Cardiomegaly  & $9834 $ $(2072, 15766)$  & $51$ $(49, 53)$ \\
Atelectasis   & $13189$ $(2511, 28171)$  & $50$ $(48, 52)$ \\

Edema         & $47$ $(12, 83)$ & $76$ $(76, 76)$ \\
Consolidation & $36$ $(2, 104)$ & $76$ $(76, 76)$\\
Cardiomegaly  & $42$ $(17, 57)$ & $75$ $(75, 75)$ \\
Atelectasis   & $80$ $(65, 98)$ & $75$ $(75, 75)$ \\


Plaintext         & $91$ & $78$ & $89$ & $85$ & $86$\\
DP-Simple, $b=10$ & $51$ & $51$ & $52$ & $52$ & $52$\\
DP-Simple, $b=20$ & $50$ & $50$ & $50$ & $50$ & $50$\\
DP-Simple, $b=30$ & $49$ & $49$ & $50$ & $51$ & $50$\\
DP-Image, $b=1$   & $60$ & $59$ & $60$ & $59$ & $60$\\
DP-Image, $b=2$   & $54$ & $50$ & $55$ & $55$ & $54$\\
DP-Image, $b=5$   & $53$ & $55$ & $51$ & $52$ & $53$\\
\name-Random      & $89$ & $75$ & $86$ & $84$ & $84$\\
\name             & $82$ & $69$ & $81$ & $78$ & $78$\\

